Equivariant homology theory and twisted Yangian

We study the convolution algebra $H^{G\times \CC^{*}}_{*}(Z)$ of $G$-equivariant homology group on the Steinberg variety of type B/C and define an algebra $\widetilde{Y}$ that maps to $H^{G\times \CC^{*}}_{*}(Z)$. The Drinfeld new realization of the twisted Yangian associated to symmetric pairs is a quotient of $\widetilde{Y}$. We also study the $G$-equivariant case and prove that the twisted Yangian is the deformation of the twisted current algebra.

==> bib.tex <==
@incollection{brion1998equivariant,
  title={Equivariant cohomology and equivariant intersection theory},
  author={Brion, Michel},
  booktitle={Representation theories and algebraic geometry},
  pages={1--37},
  year={1998},
  publisher={Springer}
}
@book{chriss2009representation,
  title={Representation theory and complex geometry},
  author={Chriss, Neil and  Ginzburg, Victor},
  year={2009},
  publisher={Springer Science \& Business Media}
}
@misc{przezdziecki2015geometric,
  title={Geometric approach to {KLR} algebras and their representation theory},
  author={Przezdziecki, Tomasz},
  year={2015}
}
@article{varagnolo2000quiver,
  title={Quiver varieties and {Yangians}},
  author={Varagnolo, Michela},
  journal={Letters in Mathematical Physics},
  volume={53},
  number={4},
  pages={273--283},
  year={2000},
  publisher={Springer}
}
@misc{fan2019equivariant,
    title={Equivariant {K-theory} approach to $\imath$-quantum groups},
    author={Zhaobing Fan and Haitao Ma and Husileng Xiao},
    year={2019},
    eprint={1911.00851},
    archivePrefix={arXiv},
    primaryClass={math.RT}
}
@misc{kamnitzer2015highest,
    title={Highest weights for truncated shifted {Yangians} and product monomial crystals},
    author={Joel Kamnitzer and Peter Tingley and Ben Webster and Alex Weekes and Oded Yacobi},
    year={2015},
    eprint={1511.09131},
    archivePrefix={arXiv},
    primaryClass={math.RT}
}
@article{nakajima1994instantons,
  title={Instantons on {ALE} spaces, quiver varieties, and {Kac-Moody} algebras},
  author={Nakajima, Hiraku},
  journal={Duke Mathematical Journal},
  volume={76},
  number={2},
  pages={365--416},
  year={1994},
  publisher={Duke University Press}
}@misc{nakajima2019coulomb,
    title={Coulomb branches of quiver gauge theories with symmetrizers},
    author={Hiraku Nakajima and Alex Weekes},
    year={2019},
    eprint={1907.06552},
    archivePrefix={arXiv},
    primaryClass={math.QA}
}
@article{li2019quiver,
  title={Quiver varieties and symmetric pairs},
  author={Li, Yiqiang},
  journal={Representation Theory of the American Mathematical Society},
  volume={23},
  number={1},
  pages={1--56},
  year={2019}
}
